First-principles molten salt phase diagrams through thermodynamic integration

Precise prediction of phase diagrams in molecular dynamics (MD) simulations is challenging due to the simultaneous need for long time scales, large length scales and accurate interatomic potentials. We show that thermodynamic integration (TI) from low-cost force fields to neural network potentials (NNPs) trained using density-functional theory (DFT) enables rapid first-principles prediction of the solid-liquid phase boundary in the model salt NaCl. We use this technique to compare the accuracy of several DFT exchange-correlation functionals for predicting the NaCl phase boundary, and find that the inclusion of dispersion interactions is critical to obtain good agreement with experiment. Importantly, our approach introduces a method to predict solid-liquid phase boundaries for any material at an ab-initio level of accuracy, with the majority of the computational cost at the level of classical potentials.

==> Makefile <==
all: main
PDFLATEX=pdflatex --halt-on-error

main: main.tex
	$(PDFLATEX) main.tex
	bibtex main
	$(PDFLATEX) main.tex
	$(PDFLATEX) main.tex

SI: SI.tex
	$(PDFLATEX) SI.tex
	#bibtex SI
	#$(PDFLATEX) SI.tex

CoverLetter: CoverLetter.tex
	$(PDFLATEX) CoverLetter.tex
	$(PDFLATEX) CoverLetter.tex

Response: Response.tex
	$(PDFLATEX) Response.tex
	$(PDFLATEX) Response.tex

Response2: Response2.tex
	$(PDFLATEX) Response2.tex
	$(PDFLATEX) Response2.tex

submit: main
	awk '{ if($$1=="\\bibliography{references}") print "\\input{main.bbl}"; else print; }' main.tex > temp.tex
	latexpand temp.tex > submit/submit.tex
	rm temp.tex


==> unused-snippets.tex <==
% ----------------------------------------------------------------------------------
Old figure 1 (overview)

\begin{figure}
\includegraphics[width=\columnwidth]{overview.pdf}
\caption{(a) Solid-liquid phase boundary of NaCl predicted by the most commonly-used classical potential matches experiment\cite{akellavaidyakennedyMeltingSodiumChloride1969} by construction at ambient pressures, but deviates from it with increasing pressure.
(b) Simulation of phase equilibria directly using coexistence methods requires large interfaces with $\sim 10^4$ atoms, in contrast to
(c) much smaller bulk simulations with $\sim 500 - 1000$ atoms required for thermodynamic integration (TI) approaches.
(d) Our general approach here is to compute free energy differences $\Delta G_{sl}$ between the phases using simple classical potentials within any approach (coexistence or TI), and then convert the predictions to first-principles quality using TI between classical and neural-network potentials (NNPs) trained to density-functional theory (DFT).}
\label{fig:overview}
\end{figure}



% ----------------------------------------------------------------------------------
Not really needed for paper, but keeping in case needed during revisions:

\begin{table} \centering
\caption{Calculation of experimental atomization energy of solid NaCl (rock salt crystal).}
\label{tab:NaCl atomization energy}
\begin{tabular}{cc}
\hline\hline
Reaction & $\Delta H$ (kJ/mol)\cite{brownLevelBornHaber2000}\\
\hline
$Na_{g}\rightarrow Na^{+}+e^{-}$ & $502$\\
$Cl_{g}+e^{-}\rightarrow Cl^{-}$ & $-355$\\
$Na^{+}+Cl^{-}\rightarrow NaCl$ & $-786$\\
$Na_{g}+\ Cl_{g}\rightarrow NaCl$ & $-639$\\
\hline
\multicolumn{2}{c}{$\Delta U=\left(  -639-PV_{gas}\right)  =-6.68eV$}\\
\hline\hline
\end{tabular}
\end{table}

%-------------------------------------------------------------------------------

Computational detail removed from main text, perhaps suitable for SI:

For the TI simulations, parameters at each $\lambda$ point were calculated separately and passed into LAMMPS, where the hybrid/overlay style was used to superimpose the relevant potentials. $\frac{dU}{d\lambda}$ was calculated using the compute ti command in LAMMPS. 
Note that in order to perform these simulations in LAMMPS artificial tether atom types must be introduced at each lattice site between steps 2 and 3 which a) must be constrained not to move over the course of the simulation by excluding them from the time integration fixes and b) must only interact with the specific ``real" atom types that would occupy each lattice site in the crystalline configuration.

%-------------------------------------------------------------------------------

\begin{algorithm}[H]
\caption{Method to predict NNP $T_m$.\label{algorithm:NNP_TI}}
\begin{algorithmic}[1]
\State With known Fumi-Tosi melting point $(P^{0},T^{0})$
\State Set temperature convergence threshold 
\State Make an initial guess for the NNP melting temperature at ambient pressure $(P^{0},T_{g})$
\State Set initial high $\Delta T$
\While 
{$\Delta T > threshold$}
    \State Run NVT TI simulations $(P^{0},T_{g})_{NNP} \rightarrow (P^{\lambda},T_{g})_{FT}$, calculate $ \Delta G_{TI}$
    \State Run Fumi-Tosi (de)compression $(P^{\lambda},T_{g}) \rightarrow (P^{0},T_{g})$, calculate $\Delta G_{C} $
    \State Run Fumi-Tosi heating (cooling) $(P^{0},T_{g}) \rightarrow (P^{0},T^{0})$, calculate $\Delta G_{H} $
    \State Use $ \Delta G_{TI} + \Delta G_{C} + \Delta G_{H}$ to obtain correction factor $\Delta T$
    \State Refine guess for NNP melting temperature $T_{g} = T_{g} + \Delta T$
\EndWhile
\State Predict converged NNP melting temperature $T^{m}_{NNP} = T_{g}$ at $P^{0}$
\end{algorithmic}
\end{algorithm}

%-------------------------------------------------------------------------------

\begin{algorithm}[H]
\caption{Method to numerically integrate Clausius-Clapeyron equation.\label{algorithm:CC}}
\begin{algorithmic} [1]
\State Set temperature convergence threshold 
\For 
{$pressures=P^{0},P^{1}, \ldots, P^{N}$}
    \State Create solid, liquid configurations at converged/known coexistence point $(P^{i},T^{i})$
    \State Calculate $dP/dT$ from $\Delta H$ and $\Delta V$
    \State Use $dP/dT$ to make a straight-line approximation for next coexistence point $(P^{i+1},T_{g})$
    \State Run compression $(P^{i},T^{i}) \rightarrow (P^{i+1},T^{i})$, calculate $\Delta G_{C} $
    \State Set initial high $\Delta T$
    \While 
    {$\Delta T > threshold$}
        \State Run heating sim $(P^{i+1},T^{i}) \rightarrow (P^{i+1},T_{g})$, calculate $\Delta G_{H} $
        \State Use $\Delta G_{C} + \Delta G_{H}$ to obtain correction factor $\Delta T$
        \State Refine guess $T_{g} = T_{g} + \Delta T$
    \EndWhile
    \State Predict converged melting temperature $T^{i+1} = T_{g}$ at $P^{i+1}$
\EndFor
\end{algorithmic}
\end{algorithm}

%-------------------------------------------------------------------------------

\begin{figure}
\includegraphics[width=\columnwidth]{cycles.pdf}
\caption{a) Thermodynamic cycle to obtain NNP coexistence point. An initial guess is made for the NNP melting point (top orange circle), from which the NNP is transformed to the Fumi-Tosi potential in an NVT ensemble, taking the system to some pressure P$^{\lambda}$. Now with particles interacting classically, a (de)compression step is run taking the system back to P$^{0}$, and a second heating (cooling) step is run to take the system to the state point (P$^{0}$, T$^{0}$), where $\Delta G_{sl}=0$ for the classical potential. The sum of these three free energies yields a correction factor for the NNP melting temperature yielding a second guess (bottom orange circle). Subsequent guesses are expected to converge upon the NNP's melting temperature. Note that this cycle must be run separately for the solid and liquid phases and a phase transition cannot occur during any of the simulations. 
b) Procedure to numerically integrate the Clausius-Clapeyron equation. $\Delta H$ and $\Delta V$ at a known coexistence point yields a straight line approximation for $T_m$ at the next selected pressure. Compression and heating steps are run from the known coexistence point to the guessed coexistence point to obtain a correction factor and refine subsequent guesses. Note that guesses at each pressure only involve iteratively running the heating simulations. }
\label{fig:cycles}
\end{figure}


%----------------------------- Old SI that was within the main text ---------------------------
\clearpage
\section{Supplementary information(?)}

\begin{itemize}
    \item Initially create separate solid and liquid configurations of atoms equilibrated at a known coexistence point $(P^{0},T^{0})$
    \item Calculate $\Delta H_{0}$ and $\Delta V_{0}$ and use the Clausius-Clapeyron equation to find $\frac{dP}{dT} $ at that state point
    \item With  pressure  as  an  independent  variable,  use  $\frac{dP}{dT}$ to make a straight-line approximation as an initial prediction for the next coexisting temperature $T_{g}$
    \item For  each  phase, run an NPT compression simulation to the new pressure while holding temperature constant $(P^{0},T^{0}) \rightarrow (P^{1},T^{0})$, and find the change in free energy due to the compression $\Delta G_{C} $ for each phase. Note that the approximation in the following equation can be made due to the unit system being used. The simulation box sizes are on the order of nanometers and while the volume of the simulation box changes as the pressure is increased, approximating the integral by using the average volume of the box over the course of the compression simulation does not change the final result much \emph{this will not stand up to scrutiny, maybe just leave the VdP integral. But that will still raise questions during a review. Ideally we should test this method out on the LJ system to see if this approximation still works in a more "evenly scaled" unit system. I guess in the LJ system in practice the $\Delta P$ term will only vary on the order of unity so the area under the curve will be very narrow, but this is still not rigorous enough} 
    \begin{equation}
        dG = -SdT + VdP \Rightarrow \Delta G_{C} = \int_{P^{0}}^{P^{1}} VdP \approx \overline{V} \Delta P
    \end{equation}
    
    \item At  the  new  pressure, run an NPT heating simulation from the original known coexistence temperature to the predicted temperature $(P^{1},T^{0}) \rightarrow (P^{1},T_{g})$ and find the difference in free energy due to heating $ \Delta G_{H} $ between the two phases. Note that since entropy cannot be directly computed through an MD simulation, $ \Delta G_{H} $ cannot be calculated independently for either phase in the heating simulations, it can only be calculated for the solid-liquid difference.
    
    \begin{equation}
        dG = -SdT + VdP \Rightarrow \Delta G_{H} = -\int_{T^{0}}^{T_{g}} SdT
    \end{equation}
    
    \begin{equation}
        dH = TdS + VdP \Rightarrow \Delta H = T \Delta S \Rightarrow \Delta S^{SL} = \frac{\Delta H^{SL}}{T}
    \end{equation}
    
    \begin{equation}
        \Delta S^{SL} = \frac{\Delta H^{SL}}{T} \Rightarrow \Delta G^{SL}_{H} = -\int_{T^{0}}^{T_{g}} \frac{\Delta H^{SL} dT} {T} 
    \end{equation}
    
    
    
    \item Use the net $\Delta G_{path}^{SL} = \Delta G_{C}^{SL} + \Delta G_{H}^{SL} $ along the pathway and $\Delta H_{0} $ at the known coexistence point to calculate a correction factor for the predicted temperature. Note that $\Delta H $ between the two phases at the known coexistence point is assumed to be equal to $\Delta H $ at the guessed point which allows us to approximate the solid-liquid entropy difference at the guessed point and obtain the correction factor as \emph{write out the intermediate steps}
    \begin{equation} 
        \Delta S_{g}^{SL} \approx \frac {\Delta H_{0}^{SL}} {T_{g}} \Rightarrow \Delta T = T_{g} \frac {\Delta G_{path}^{SL}}{ \Delta H_{0}^{SL}}  
    \end{equation}
    
    
    
    % TS: this assumption is the key reason why these algorithms work right? That the enthalpy difference at the known coexistence point will be roughly equal to the enthalpy difference at any other coexistence point?
    \item Repeat heating simulations at $P^{1}$ until the temperature correction factors converge
    \item Calculate $\frac{dP}{dT}$ at the new converged coexistence point, make an initial straight line approximation for the melting temperature at the next pressure, and repeat
\end{itemize}

